Simultaneous Tensor Completion and Denoising by Noise Inequality Constrained Convex Optimization

Tensor completion is a technique of filling missing elements of the incomplete data tensors. It being actively studied based on the convex optimization scheme such as nuclear-norm minimization. When given data tensors include some noises, the nuclear-norm minimization problem is usually converted to the nuclear-norm `regularization' problem which simultaneously minimize penalty and error terms with some trade-off parameter. However, the good value of trade-off is not easily determined because of the difference of two units and the data dependence. In the sense of trade-off tuning, the noisy tensor completion problem with the `noise inequality constraint' is better choice than the `regularization' because the good noise threshold can be easily bounded with noise standard deviation. In this study, we tackle to solve the convex tensor completion problems with two types of noise inequality constraints: Gaussian and Laplace distributions. The contributions of this study are follows: (1) New tensor completion and denoising models using tensor total variation and nuclear-norm are proposed which can be characterized as a generalization/extension of many past matrix and tensor completion models, (2) proximal mappings for noise inequalities are derived which are analytically computable with low computational complexity, (3) convex optimization algorithm is proposed based on primal-dual splitting framework, (4) new step-size adaptation method is proposed to accelerate the optimization, and (5) extensive experiments demonstrated the advantages of the proposed method for visual data retrieval such as for color images, movies, and 3D-volumetric data.

==> mathdef.tex <==
%#!platex sotsuron.tex
%%% 論文内で使う記号はマクロとして定義しておきましょう．
%%% あとで，使う文字を変更するのも簡単です.

%\newtheorem{definition}{ \ \ Definition}[section]
%\newtheorem{theorem}{ \ \ Theorem}[section]
%\newtheorem{nature}{ \ \ Nature}[section]
%\newtheorem{lemma}{ \ \ Lemma}[section]
%\newtheorem{expectation}{ \ \ 予想}[section]
%\newtheorem{algorithm}{ \ \ アルゴリズム}[section]
%\newtheorem{proposition}{{\bf \ \ 命題}}[section]
%\newtheorem{corollary}{{\bf \ \ 系}}[section]
%\newtheorem{example}{{\bf \ \ 例}}[section]
%\newtheorem{theoremproof}{{\bf \ \ (証明)}}
%\renewcommand{\thetheoremproof}{}
%\newtheorem{lemmaproof}{{\bf \ \ (証明)}}
%\renewcommand{\thelemmaproof}{}

%\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\dx}{\mathrm d \bm x}

\newcommand{\inp}[2]{ \left\langle #1 , #2 \right\rangle }

\newcommand{\define}{\stackrel{\mathrm{def}}{=}}
\newcommand{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\text{\rm minimize\ \ \ \ }}
\newcommand{\maximize}{\text{\rm maximize\ \ \ \ }}
\newcommand{\st}{\text{\rm subject to\ \ \ }}
\renewcommand{\max}{\mathop{\mathrm{max}}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\trace}[1]{\mathrm{tr}(#1)}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\trans}[1]{#1^\top}
\newcommand{\unorm}[1]{\left\|#1\right\|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\unorms}[1]{\unorm{#1}^2}
\newcommand{\inner}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\atan}{\mathop{\mathrm{arctan}}}

%%%実験用
\newcommand{\Wx}{W_x}
\newcommand{\Wy}{W_y}

%%% サンプル数の変数
\newcommand{\sampj}{i}
\newcommand{\sampmax}{M}
%%% LMF用
\newcommand{\y}{\psi}
\newcommand{\xy}{(x,y)}
\newcommand{\Dxy}{D(x,y)}
\newcommand{\hxy}{h(x,y)}
\newcommand{\Lorg}{L}
\newcommand{\Lrxy}{\Lr (x,y)}
\newcommand{\Loxy}{\Lo (x,y)}
\newcommand{\thetax}{\theta_\mathrm{x}}
\newcommand{\thetay}{\theta_\mathrm{y}}
\newcommand{\thetarm}{\theta}
\newcommand{\fx}{f_\mathrm{x}}
\newcommand{\hatfx}{\hat{\fx}}
\newcommand{\fy}{f_\mathrm{y}}
\newcommand{\hatfy}{\hat{\fy}}
\newcommand{\Trxy}{\Tr (x,y)}
\newcommand{\Toxy}{\To (x,y)}
\newcommand{\phixy}{\phi (x,y)}
\newcommand{\Tdelta}{T_\delta}
\newcommand{\Tdelxy}{\Tdelta (x,y)}
\newcommand{\pdelta}{2\pi\fx x+2\pi\fy y}
\newcommand{\hatpdelta}{2\pi\hatfx x+2\pi\hatfy y}
\newcommand{\Pxy}{P(x,y)}


\newcommand{\xj}{x_\sampj}
\newcommand{\yj}{y_\sampj}
\newcommand{\pdeltaj}{2\pi\fx \xj+2\pi\fy \yj}
\newcommand{\Tdxy}{\Td (x,y)}
\newcommand{\bdxy}{\bd (x,y)}
\newcommand{\bcxy}{\bc (x,y)}
\newcommand{\bsxy}{\bs (x,y)}
\newcommand{\mphixy}{m_\phi (x,y)}

\newcommand{\goxy}{\go (x,y)}
\newcommand{\gxy}{g(x,y)}
\newcommand{\gxyj}{g(\xj,\yj)}
\newcommand{\gj}{g_\sampj}
\newcommand{\phic}{\varphi_c}
\newcommand{\phis}{\varphi_s}
\newcommand{\phicxy}{\phic (x,y)}
\newcommand{\phisxy}{\phis (x,y)}
\newcommand{\phicj}{\phic (\xj,\yj)}
\newcommand{\phisj}{\phis (\xj,\yj)}
\newcommand{\phistar}{\phi ^\star}
\newcommand{\xyjM}{\{(\xj,\yj)\}_{\sampj=1}^\sampmax}

\newcommand{\hatbd}{\widehat{b}_d}
\newcommand{\hatbc}{\widehat{b}_c}
\newcommand{\hatbs}{\widehat{b}_s}
\newcommand{\phihat}{\widehat{\phi}}
\newcommand{\hatg}{\widehat{g}}

\newcommand{\vecg}{\bm{g}}
\newcommand{\A}{\bm{\mathrm{A}}}
%%%filmLMF
\newcommand{\Ljxy}{\Lj(x,y)}
\newcommand{\TDxy}{T_D(x,y)}
\newcommand{\Tjxy}{T_j(x,y)}
\newcommand{\mucxy}{\muc (x,y)}
\newcommand{\musxy}{\mus (x,y)}
\newcommand{\ze}{\zeta}
\newcommand{\zezetaxy}{1+\keisu^2-2\keisu\cos(2k\kussetui\Dxy)}
\newcommand{\zezeta}{1+\keisu^2-2\keisu\cos(2k\kussetui\D)}
\newcommand{\zexy}{\zeta(D(x,y))}
\newcommand{\zeD}{\zeta(D)}
\newcommand{\zexyi}{\zeta(D(x_i,y_i))}
\newcommand{\Tzxy}{\Tz (x,y)}
\newcommand{\Tixy}{\Ti (x,y)}
\newcommand{\hs}{\h_\mathrm{s}}
\newcommand{\hatD}{\hat{D}}
\newcommand{\hatDnew}{\hatD_\mathrm{new}}
\newcommand{\hatDnewfilt}{\hatD_\mathrm{newfilt}}
\newcommand{\hatDfilt}{\hatD_\mathrm{filt}}
\newcommand{\hath}{\hat{\h}}
\newcommand{\hathnew}{\hat{\h}_\mathrm{new}}
\newcommand{\hathnewfilt}{\hat{\h}_\mathrm{newfilt}}
\newcommand{\hathfilt}{\hat{\h}_\mathrm{filt}}
\newcommand{\haths}{\hat{\hs}}

%%% speed up
\newcommand{\Comp}{\mathop{\it Comp}}
\newcommand{\comp}{\mathop{\it comp}}
\newcommand{\qq}{\qquad : \qquad}
\renewcommand{\S}{\bm{\mathrm{S}}}
\newcommand{\T}{\bm{\mathrm{T}}}
\renewcommand{\t}{\bm{t}}
\newcommand{\hatb}{\hat{\bm{b}}}
%%error
\newcommand{\Delbd}{\Delta\bd}
\newcommand{\Delbc}{\Delta\bc}
\newcommand{\Delbs}{\Delta\bs}
\newcommand{\Delgxi}{\Delta g(x_i)}
\newcommand{\Delg}{\Delta g}
\newcommand{\Delphixi}{\Delta \phi _i}
\newcommand{\Delphi}{\Delta \phi}
\newcommand{\bcz}{\bc}
\newcommand{\bsz}{\bs}
\newcommand{\Delalmax}{\Delta\alpha_{\mathrm{max}}}
\newcommand{\Delalmin}{\Delta\alpha_{\mathrm{min}}}
\newcommand{\sumalli}{\sum_{i=-n}^n}
\newcommand{\sumi}{\sum_{i=1}^n}
\newcommand{\sdphi}{\sin \Delphixi}
\newcommand{\ssdphi}{\sin^2 \frac{\Delphixi}{2}}
%%%位相シフト法(小川)より
\newcommand{\eq}[1]{式(\ref{#1})}
\newcommand{\eqs}[2]{式(\ref{#1})，(\ref{#2})}
\newcommand{\eqss}[3]{式(\ref{#1})，(\ref{#2})，(\ref{#3})}
\newcommand{\eqsss}[4]{Eqs.\,(\ref{#1}), (\ref{#2}), (\ref{#3}), (\ref{#4})}
\newcommand{\eqssss}[5]{式(\ref{#1})，(\ref{#2})，(\ref{#3})，(\ref{#4})，(\ref{#5})}
\newcommand{\eqsssss}[6]{式(\ref{#1})，(\ref{#2})，(\ref{#3})，(\ref{#4})，(\ref{#5})，(\ref{#6})}
\newcommand{\eqssssss}[7]{式(\ref{#1})，(\ref{#2})，(\ref{#3})，(\ref{#4})，(\ref{#5})，(\ref{#6})，(\ref{#7})}

\newcommand{\ar}{a_{\mathrm{ref}}}
\newcommand{\ao}{a_{\mathrm{obj}}}
\newcommand{\az}{a_0}
\newcommand{\ai}{a_1}
\newcommand{\aii}{a_2}
\newcommand{\aj}{a_j}

\newcommand{\bd}{b_\mathrm{d}}
\newcommand{\bc}{b_\mathrm{c}}
\newcommand{\bs}{b_\mathrm{s}}
\newcommand{\bds}{b_\mathrm{d}^\star}
\newcommand{\bcs}{b_\mathrm{c}^\star}
\newcommand{\bss}{b_\mathrm{s}^\star}
\newcommand{\bdh}{\widehat{b}_\mathrm{d}}
\newcommand{\bch}{\widehat{b}_\mathrm{c}}
\newcommand{\bsh}{\widehat{b}_\mathrm{s}}

\newcommand{\gs}{g^\star}

\newcommand{\hensu}{\xi}
\newcommand{\karix}{x}
\newcommand{\karir}{r}
\newcommand{\karia}{b_1}
\newcommand{\karib}{b_2}
\newcommand{\karic}{b_3}
\newcommand{\karid}{b_4}
\newcommand{\karip}{p}
\newcommand{\kariq}{q}

\newcommand{\ci}{c_1}
\newcommand{\cii}{c_2}
\newcommand{\ciii}{c_3}
\newcommand{\civ}{c_4}
\newcommand{\cv}{c_5}
\newcommand{\cvi}{c_6}
\newcommand{\cvii}{c_7}


\newcommand{\bfb}{\mbox{\boldmath $b$}}

\newcommand{\keisu}{\rho _1 } % 'keisu'は反射係数，透過係数の係数を表す．
\newcommand{\keisui}{\eta _1}
\newcommand{\keisuii}{\eta _c}

\newcommand{\keisua}{\rho _{\mathrm{01}}}      % 膜の表面反射係数
\newcommand{\keisuaa}{\rho _{\mathrm{10}}}     % 膜の表面反射係数
\newcommand{\keisut}{\tau _{\mathrm{01}}}      % 膜の表面透過係数
\newcommand{\keisutt}{\tau _{\mathrm{10}}}     % 膜の表面透過係数
\newcommand{\keisus}{\rho _{\mathrm{12}}}      % 膜の裏面反射係数
\newcommand{\keisuss}{\rho}                    % 膜なしの表面反射係数
\newcommand{\keisuasi}{\eta _{as1}}   % 膜の反射係数
\newcommand{\keisuasii}{\eta _{as2}}  % 膜の反射係数

\newcommand{\keisurr}{\gamma}
\newcommand{\keisuo}{\tau _{\mathrm{BS}}}      % ビームスプリッタの透過係数
\newcommand{\keisur}{\rho _{\mathrm{BS}}}      % ビームスプリッタの反射係数
\newcommand{\keisum}{\rho _{\mathrm{ref}}}     % 参照鏡の反射係数
\newcommand{\keisue}{\eta _{\mathrm{e}}}       % 装置係数
% \newcommand{\keisub}{\eta _b} 
\newcommand{\keisub}{\keisuo ^2} 
\newcommand{\keisud}{\alpha} 
\newcommand{\keisuh}{\beta} 

% \newcommand{\tkeisu}{\gamma}
% \newcommand{\tkeisur}{\gamma _r}
% \newcommand{\tkeisuz}{\gamma _0}
% \newcommand{\tkeisui}{\gamma _1}
% \newcommand{\tkeisuii}{\gamma _2}
% \newcommand{\tkeisuj}{\gamma _j}

\newcommand{\kussetui}{n_1} 
\newcommand{\kussetuii}{n_2} 

\newcommand{\Lr}{L_{\mathrm{ref}}}
\newcommand{\Lo}{L_{\mathrm{obj}}}
\newcommand{\Lz}{L_0}
\newcommand{\Li}{L_1}
\newcommand{\Lj}{L_j}

\newcommand{\Td}{T_\mathrm{d}}
\newcommand{\TD}{T_\mathrm{D}}
\newcommand{\Tr}{T_{\mathrm{ref}}}
\newcommand{\To}{T_{\mathrm{obj}}}
\newcommand{\Tz}{T_0}
\newcommand{\Ti}{T_1}
\newcommand{\Tj}{T_j}

\newcommand{\ys}{\psi_\mathrm{s}}
\newcommand{\yr}{\psi_{\mathrm{ref}}}
\newcommand{\yo}{\psi_{\mathrm{obj}}}
\newcommand{\yjj}{\psi_j}
\newcommand{\jj}{j\; \left(j=0,1,\dots\right)}

\newcommand{\gr}{g_{\mathrm{ref}}}
\newcommand{\go}{g_{\mathrm{obj}}}
% \newcommand{\gj}{g_j}
\newcommand{\kansokugj}{\widehat{g}_\sampj}
\newcommand{\gjM}{\{g_\sampj\}_{\sampj=0}^{\sampmax-1}}
\newcommand{\h}{h}
\newcommand{\zp}{h} %以前はhをzpと書いていた
\newcommand{\D}{D}
\newcommand{\zj}{z_\sampj}
\newcommand{\zjM}{\{z_\sampj\}_{\sampj=0}^{\sampmax-1}}
\newcommand{\thetaj}{\frac{2\pi}{M}\sampj}

\newcommand{\lam}{\lambda}
\newcommand{\mus}{\mu_\mathrm{s}}
\newcommand{\muc}{\mu_\mathrm{c}}
%
\newcommand{\md}{m_\mathrm{d}}
\newcommand{\mz}{m_\mathrm{h}}
\newcommand{\mh}{m_\mathrm{h}}
%\newcommand{\sumnN}{\sum_{n=1}^{N}}
%\newcommand{\summN}{\sum_{m=1}^{N}}
%\newcommand{\summM}{\sum_{m=1}^{M}}
%\newcommand{\sumiN}{\sum_{i=1}^{N}}
%\newcommand{\sumlL}{\sum_{l=1}^{L}}
%
%\newcommand{\xnN}{\{\bfxn\}_{n=1}^{N}}
%\newcommand{\xmM}{\{\bfxm\}_{m=1}^{M}}
%\newcommand{\ynN}{\{\yn\}_{n=1}^{N}}
%\newcommand{\ymM}{\{\ym\}_{m=1}^{M}}
%\newcommand{\xnynN}{\{\bfxn, \yn\}_{n=1}^{N}}
%\newcommand{\xmymM}{\{\bfxm, \ym\}_{m=1}^{M}}
%\newcommand{\xilL}{\{\xi _l\}_{l=1}^{L}}
%\newcommand{\unN}{\{u_n\}_{n=1}^{N}}
%\newcommand{\umM}{\{u_m\}_{m=1}^{M}}
%\newcommand{\usnN}{\{u_n^*\}_{n=1}^{N}}
%\newcommand{\vnN}{\{v_n\}_{n=1}^{N}}
%\newcommand{\vsnN}{\{v_n^*\}_{n=1}^{N}}
%\newcommand{\unusnN}{\{\un,\usn\}_{n=1}^{N}}
%\newcommand{\vnvsnN}{\{\vn,\vsn\}_{n=1}^{N}}
%\newcommand{\wnN}{\{\wn\}_{n=1}^{N}}
%\newcommand{\wmM}{\{\wm\}_{m=1}^{M}}

%
%\newcommand{\inpro}[2]{\langle#1, #2\rangle}
%\newcommand{\inprob}[2]{\left\langle#1, #2\right\rangle}
%\newcommand{\spro}[2]{#1\otimes\overline{#2}}
%\newcommand{\nrm}[1]{\parallel #1 \parallel}
%
%\newcommand{\dps}{\displaystyle}
%\newcommand{\sinc}{{\rm sinc}}
%\newcommand{\qed}{\mbox{}\hfill\hbox{\rule{6pt}{6pt}}}

% \newcommand{\Uii}{U_2}
% \newcommand{\Vii}{V_2}

%%%%%%%%%
%
%\newcommand{\mathbbC}{\mathbb{C}}
%\newcommand{\mathbbE}{\mathbb{E}}
%\newcommand{\mathbbN}{\mathbb{N}}
%\newcommand{\mathbbR}{\mathbb{R}}
%
%\newcommand{\boldzero}{{\boldsymbol{0}}}
%\newcommand{\boldone}{{\boldsymbol{1}}}
%
%\newcommand{\boldA}{{\boldsymbol{A}}}
%\newcommand{\boldB}{{\boldsymbol{B}}}
%\newcommand{\boldC}{{\boldsymbol{C}}}
%\newcommand{\boldD}{{\boldsymbol{D}}}
%\newcommand{\boldE}{{\boldsymbol{E}}}
%\newcommand{\boldF}{{\boldsymbol{F}}}
%\newcommand{\boldG}{{\boldsymbol{G}}}
%\newcommand{\boldH}{{\boldsymbol{H}}}
%\newcommand{\boldI}{{\boldsymbol{I}}}
%\newcommand{\boldJ}{{\boldsymbol{J}}}
%\newcommand{\boldK}{{\boldsymbol{K}}}
%\newcommand{\boldL}{{\boldsymbol{L}}}
%\newcommand{\boldM}{{\boldsymbol{M}}}
%\newcommand{\boldN}{{\boldsymbol{N}}}
%\newcommand{\boldO}{{\boldsymbol{O}}}
%\newcommand{\boldP}{{\boldsymbol{P}}}
%\newcommand{\boldQ}{{\boldsymbol{Q}}}
%\newcommand{\boldR}{{\boldsymbol{R}}}
%\newcommand{\boldS}{{\boldsymbol{S}}}
%\newcommand{\boldT}{{\boldsymbol{T}}}
%\newcommand{\boldU}{{\boldsymbol{U}}}
%\newcommand{\boldV}{{\boldsymbol{V}}}
%\newcommand{\boldW}{{\boldsymbol{W}}}
%\newcommand{\boldX}{{\boldsymbol{X}}}
%\newcommand{\boldY}{{\boldsymbol{Y}}}
%\newcommand{\boldZ}{{\boldsymbol{Z}}}
%
%\newcommand{\bolda}{{\boldsymbol{a}}}
%\newcommand{\boldb}{{\boldsymbol{b}}}
%\newcommand{\boldc}{{\boldsymbol{c}}}
%\newcommand{\boldd}{{\boldsymbol{d}}}
%\newcommand{\bolde}{{\boldsymbol{e}}}
%\newcommand{\boldf}{{\boldsymbol{f}}}
%\newcommand{\boldg}{{\boldsymbol{g}}}
%\newcommand{\boldh}{{\boldsymbol{h}}}
%\newcommand{\boldi}{{\boldsymbol{i}}}
%\newcommand{\boldj}{{\boldsymbol{j}}}
%\newcommand{\boldk}{{\boldsymbol{k}}}
%\newcommand{\boldl}{{\boldsymbol{l}}}
%\newcommand{\boldm}{{\boldsymbol{m}}}
%\newcommand{\boldn}{{\boldsymbol{n}}}
%\newcommand{\boldo}{{\boldsymbol{o}}}
%\newcommand{\boldp}{{\boldsymbol{p}}}
%\newcommand{\boldq}{{\boldsymbol{q}}}
%\newcommand{\boldr}{{\boldsymbol{r}}}
%\newcommand{\bolds}{{\boldsymbol{s}}}
%\newcommand{\boldt}{{\boldsymbol{t}}}
%\newcommand{\boldu}{{\boldsymbol{u}}}
%\newcommand{\boldv}{{\boldsymbol{v}}}
%\newcommand{\boldw}{{\boldsymbol{w}}}
%\newcommand{\boldx}{{\boldsymbol{x}}}
%\newcommand{\boldy}{{\boldsymbol{y}}}
%\newcommand{\boldz}{{\boldsymbol{z}}}
%
%\newcommand{\boldalpha}{{\boldsymbol{\alpha}}}
%\newcommand{\boldbeta}{{\boldsymbol{\beta}}}
%\newcommand{\boldepsilon}{{\boldsymbol{\varepsilon}}}
%\newcommand{\boldxi}{{\boldsymbol{\xi}}}
%\newcommand{\boldmu}{{\boldsymbol{\mu}}}
%\newcommand{\boldomega}{{\boldsymbol{\omega}}}
%\newcommand{\boldLambda}{{\boldsymbol{\Lambda}}}
%
%\newcommand{\calD}{{\mathcal D}}
%\newcommand{\calL}{{\mathcal L}}
%\newcommand{\calM}{{\mathcal M}}
%\newcommand{\calN}{{\mathcal N}}
%\newcommand{\calO}{{\mathcal O}}
%\newcommand{\calP}{{\mathcal P}}
%\newcommand{\calR}{{\mathcal R}}
%\newcommand{\calS}{{\mathcal S}}
%\newcommand{\calH}{{\mathcal H}}
%\newcommand{\calX}{{\mathcal X}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmy}{\mathrm{y}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

